The thermal-radiative wind in the neutron star low mass X-ray binary GX 13+1

We fit the observed high ionisation X-ray absorption lines in the neutron star binary GX13+1 with a full simulation of a thermal-radiative wind. This uses a radiation hydrodynamic code coupled to Monte Carlo radiation transfer to compute the observed line profiles from Hydrogen and Helium-like iron and Nickel, including all strong K{\alpha} and K{\beta} transitions. The wind is very strong as this object has a very large disc and is very luminous. The absorption lines from Fe K{\alpha} are strongly saturated as the ion columns are large, so the line equivalent widths (EWs) depend sensitively on the velocity structure. We additionally simulate the lines including isotropic turbulence at the level of the azimuthal and radial velocities. We fit these models to the Fe xxv and xxvi absorption lines seen in the highest resolution Chandra third order HETGS data. These data already rule out the addition of turbulence at the level of the radial velocity of ~500 km/s. The velocity structure predicted by the thermal-radiative wind alone is a fairly good match to the observed profile, with an upper limit to additional turbulence at the level of the azimuthal velocity of ~100 km/s. This gives stringent constraints on any remaining contribution from magnetic acceleration.

==> README <==
% readme.txt
%
% MNRAS journal LaTeX package
% v3.0 for LaTeX 2e
%
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `author-maintained'.
% 
% The Current Maintainer of this work is: Royal Astronomical Society,
% MNRAS Editorial Office, who can be contacted on mn@ras.org.uk
%
% This work consists of all the files listed in readme.txt
%
%
% Last updated 22 May 2015
%
% Copyright (C) Royal Astronomical Society 2015, Blackwell Science 2001,
% Cambridge University Press 1994
%
% See each file for a detailed author list and change log.
%
% This package consists of the following files:

readme.txt          This file

mnras.cls           MNRAS LaTeX document class
mnras.bst           MNRAS BibTeX style

mnras_guide.tex     User guide, LaTeX format
mnras_guide.pdf     User guide, PDF format
mnras_template.tex  A simple template paper

example.eps         An example image used in the guide
example.png         An example image used in the guide
example.ps          An example image used in the guide

legacy\legacy.txt   Description of the legacy releases
legacy\mn2e.cls     v2.2 of mn2e.cls (deprecated)
legacy\mn2e.bst     v1.1b of mn2e.bst (deprecated)


% Disclaimer:
%
% This LaTeX package is provided free to the community in the hope that it
% assists them in preparing papers for the journal Monthly Notices of the
% Royal Astronomical Society.
% The files are provided 'as-is' with no guarantee of their suitability,
% freedom from errors or omissions, or compatibility with any software.
% The Royal Astronomical Society cannot provide user support for this package,
% LaTeX, or for any other software.
% Authors are free to use other styles or programmes if they wish.
% Please see the journal instructions to authors for guidance.
% This disclaimer is in addition to the No Warranty section of the licence,
% at the link given above.
